Tight Bound for the Number of Distinct Palindromes in a Tree

For an undirected tree with $n$ edges labelled by single letters, we consider its substrings, which are labels of the simple paths between pairs of nodes. We prove that there are $O(n^{1.5})$ different palindromic substrings. This solves an open problem of Brlek, Lafreni\`ere, and Proven\c{c}al (DLT 2015), who gave a matching lower-bound construction. Hence, we settle the tight bound of $\Theta(n^{1.5})$ for the maximum palindromic complexity of trees. For standard strings, i.e., for paths, the palindromic complexity is $n+1$. We also propose $O(n^{1.5} \log{n})$-time algorithm for reporting all distinct palindromes in an undirected tree with $n$ edges.

==> _fig_example.tex <==

\tikzstyle{st} = [draw, circle, fill=black, minimum size = 5pt, inner sep = 0 pt, color=black]
\tikzstyle{stred} = [draw, circle, fill=black, minimum size = 6pt, inner sep = 0 pt, color=red]
\tikzstyle{lred} = [draw, ultra thick, color=red]
%
\node [st] (n1) at (0,1) {};
\node [st] (n2) at (0,3) {};
%
\node [st] (n3) at (2,0) {};
\node [st] (n4) at (2,2) {};
%
\node [st] (n5) at (3,3.5) {};
%
\node [st] (n6) at (4,1) {}; %% root
%
\node [st] (n7) at (5,2.1) {};
\node [st] (n8) at (5.5,0) {};
%
\node [st] (n9) at (6.5,3) {};
%
\node [st] (n10) at (6.8,1.5) {};
%
\node [st] (n11) at (8.3,1.6) {};
%
\node [st] (n12) at (7, -0.5) {};
\node [st] (n13) at (8.5, 0) {};
%
\draw (n1)-- node[midway,above] {$c$} (n3);
\draw (n2)-- node[midway,above] {$a$} (n4);
\draw (n4)-- node[midway,left] {$b$} (n5);
\draw (n3)-- node[midway,above] {$b$} (n6);
\draw (n4)-- node[midway,above] {$c$} (n6);
\draw (n6)-- node[midway,above] {$a$} (n7);
\draw (n6)-- node[midway,above] {$c$} (n8);
\draw (n7)-- node[midway,above] {$a$} (n9);
\draw (n9)-- node[midway,right] {$c$} (n10);
\draw (n10)-- node[midway,above] {$a$} (n11);
\draw (n8)-- node[midway,above] {$b$} (n12);
\draw (n12)-- node[midway,above] {$c$} (n13);


==> _fig_lower_bound.tex <==
\begin{tikzpicture}
  \tikzstyle{n}=[draw,shape=circle,minimum size=1mm,inner sep=0pt,outer sep=0pt,fill=black]
  \foreach \i in {0, ..., 8} {
    \node[n] at (\i,0) {};
    \node[n] at (\i,-1.5) {};
    \draw (\i,0) -- (\i, -1.5) node[midway,right] {$1^p$};
  }
  \foreach \i in {0, ..., 7} {
    \draw (\i,0) -- +(1, 0);
  }
  \node at (0.5,0) [above] {$0^{b_1}$};
  \node at (1.5,0) [above] {$0^{b_2}$};
  \node at (2.5,0) [above] {$0^{b_3}$};
  \node at (3.5,0) [above] {$0^{b_4}$};
  \node at (4.5,0) [above] {$0^{b_5}$};
  \node at (5.5,0) [above] {$0^{b_6}$};
  \node at (6.5,0) [above] {$\cdots$};
  \node at (7.5,0) [above] {$0^{b_{p-2}}$};

\end{tikzpicture}
